An Efficient Closed-Form Method for Optimal Hybrid Force-Velocity Control

This paper derives a closed-form method for computing hybrid force-velocity control. The key idea is to maximize the kinematic conditioning of the mechanical system, which includes a robot, free objects, a rigid environment and contact constraints. The method is complete, in that it always produces an optimal/near optimal solution when a solution exists. It is efficient, since it is in closed form, avoiding the iterative search of previous work. We test the method on 78,000 randomly generated test cases. The method outperforms our previous search-based technique by being from 7 to 40 times faster, while consistently producing better solutions in the sense of robustness to kinematic singularity. We also test the method in several representative manipulation experiments.

==> sections/ACKNOWLEDGMENT.tex <==
% !TEX root = ../ICRA19Hybrid.tex

\section*{ACKNOWLEDGMENT}
We would like to thank Hongkai Dai, Nikil Chavan-Dafle and Fran{\c{c}}ois Hogan for helpful discussions and suggestions.
